It's just a matter of perspective(s): Crowd-Powered Consensus Organization of Corpora

We study the problem of organizing a collection of objects - images, videos - into clusters, using crowdsourcing. This problem is notoriously hard for computers to do automatically, and even with crowd workers, is challenging to orchestrate: (a) workers may cluster based on different latent hierarchies or perspectives; (b) workers may cluster at different granularities even when clustering using the same perspective; and (c) workers may only see a small portion of the objects when deciding how to cluster them (and therefore have limited understanding of the "big picture"). We develop cost-efficient, accurate algorithms for identifying the consensus organization (i.e., the organizing perspective most workers prefer to employ), and incorporate these algorithms into a cost-effective workflow for organizing a collection of objects, termed ORCHESTRA. We compare our algorithms with other algorithms for clustering, on a variety of real-world datasets, and demonstrate that ORCHESTRA organizes items better and at significantly lower costs.

==> prelim.tex <==
%!TEX root = sig-alternate.tex

The problem of clustering can be stated as,\ayush{cite} 
\begin{quote}
Partition a set of items into groups such that items within a group are similar, while items from different groups are dissimilar. 
\end{quote}
This understanding of clustering is underspecified - the similarity function and the granularity of partitioning are left undefined, and are often problem specific. Clustering research has focused on these issues, with techniques such as K-Means Clustering, Hierarchical Clustering, Spectral Clustering, etc. and similarity functions tailored to the items in question (\karan{examples}). Humans are considered a benchmark in clustering data, with \cite{ng2002spectral} stating of their technique ``the algorithm reliably finds clusterings consistent with what a human would have chosen". We formalize this notion of human clustering below, as the \textsc{Consensus-Find} problem:



%Previously, clustering has been defined as 
%
%``Given a task of items, \textsc{Clustering} is the task of grouping them in such a way that objects in the same group are similar"
%
%There are a number of factors that make the above definition insufficient. For a start, how many groups are the items clustered into? Further, how to we define the `similarity' between two items -- a tiger and a lion are `similar' in that they both belong to the cat family but are yet `distinct' in being separate species. 
%%In fact, most authors define clustering in terms of the underlying criteria for grouping items together -- ``\textit{clusters of objects are formed so that objects within a cluster have high similarity in comparison to one another, but are very dissimilar to objects in other clusters}". 
%
%The problem of defining clustering is even more vague when the data is complex (for example images) - the underlying similarity judgements are subjective and are ill-defined. 
%
%This open-endedness in defining clustering stems from the fact that clustering is largely exploratory in nature, as opposed to confirmatory analysis. However, such a vague description does little to identify the problem at hand, allowing for different solutions which are hard to compare, each optimizing for a different objective. As a work-around, we adopt the following generic definition of crowdsourced clustering:

\begin{problem}[{\bf Consensus-Find Problem}]
%Given a set of items, \textsc{Human-Clustering} is the problem of organizing them into meaningful groups. These groups should have maximum likelihood, in the sense that a human should have the maximum probability of coming up with these groups, if they had complete information about the entire dataset.
Given a set of items and worker responses, \textsc{Consensus-Find} is the problem of finding a consensus clustering of the data. For a worker who has information about the entire dataset, the probability of coming up with this organization should be maximum. 
\end{problem}

%\karan{Aditya's introduction makes this redundant.}
%A solution to the \textsc{Consensus-Find} problem has to tackle the following challenges:
%\begin{enumerate}
%\item Individuals cannot cluster the entire set of items in one go. Large corpora often contain thousands of items, and it is unreasonable to expect a single human to look at the entire dataset and organize it into clusters. They can only look at small subsets of the data and provide clustering for these subsets.
%\item Different humans may organize the data in different ways. As we saw previously, different humans can choose different \textit{dimensions} to cluster a set of items. Even among the workers clustering on the same dimension, people choose different {\it granularities} to organize the data. 



%\begin{figure}[hbtp]
%\centering
%\includegraphics[scale=0.3]{../figs/different_clusters.png}
%\caption{\label{fig:different_clusters}Subjective nature of Clustering}
%\end{figure}

%\end{enumerate}

In this work, we utilize the fact that humans are competent at making similarity judgments, but may do so in different ways, depending on how they perceive the data given to them. As our pilot experiment demonstrated, workers rarely make mistakes \emph{w.r.t.} the organization they have in mind, so it is essential to understand these differences in organization, rather than directly seeking consensus amongst different workers, and labeling deviations from this consensus as `mistakes'.

%Moreover, even if humans were to cluster by shape, different humans can choose to group them as \{{\tt Quadrilaterals}, {\tt Triangles}, {\tt Ellipses}\} or as \{{\tt Polygons}, {\tt Ellipses}\}. To study this behavior experimentally, we asked 20 workers on Amazon Mechanical Turk to cluster 25 images -- Each image had a random shape, color and size from a fixed set. The task layout and the images are shown in Figure~\ref{fig:prelim_task}. 

%\begin{figure}[hbtp]
%\centering
%\includegraphics[scale=0.1]{../figs/img2.png}
%\caption{\label{fig:prelim_task}Subjective nature of Clustering}
%\end{figure}

%Workers organized the data on different dimensions - `shape' (85\%), `color' (10\%) and `size' (5\%). Even among the workers who chose to cluster on {\it shape}, the organization varied among \{{\tt Polygons}, {\tt Ellipses}\}, \{{\tt Rectangles}, {\tt Triangles}, {\tt Ellipses}\}, \{{\tt Triangles}, {\tt non-Triangles}\}, \{{\tt Square}, {\tt Rectangle}, {\tt Circle}, {\tt Ellipse}, {\tt Equilateral Triangles}, {\tt Scalene Triangle}\}. Note that the number of clusters in each of these organizations was also different. 
%
%Even though the data chosen for this exercise was artificially created and was relatively easy to cluster, we make the following observations about workers' behavior. (1) The workers were largely consistent with the organization that they chose - the cluster meant for {\tt Rectangles} had all rectangles. This was true for all workers except one, who put a square into {\tt Triangle} cluster, and (2) There were no cases where workers mixed two different modes of organization, i.e, no worker created clusters on shape and color \{{\tt red triangles}, {\tt green triangles}...\}. Next, we use these observations to formalize a worker behavior model.

%\subsection{Worker Behavior}
%We first introduce some notation that will help us in building other ideas later. 
%
%
%
%Each cluster in a meaningful clustering can be associated with an underlying latent {\it concept}. For example, in Figure~\ref{fig:prelim_task}, the clusters (from left to right) represent the concepts {\tt Rectangles}, {\tt Ellipses} and {\tt Triangles}. Intuitively, a {\it concept} is a representation of a cluster. A concept can thus be equivalently represented by the set of items in the dataset that are instances of that concept. We also include a universal concept {\tt Universe} which represents the cluster of all items in the dataset. 
%
%Very often, these concepts have subset relationships among them - {\tt Equilateral triangles} is a subset of {\tt Triangles}. More formally, concept $A$ is a subset of another concept $B$ (denoted $A\subset B$) if every item that is an instance of $A$ in the dataset is also an instance of $B$. Note that every concept is a subset of {\tt Universe}.
%Different concepts can be organized into a directed acyclic graph on this subset relationship. We call this DAG a {\it concept-DAG}.
%
%
%\begin{definition}{\bf Concept-DAG}
%A {\sc Concept-DAG} is an organization of concepts into a directed acyclic graph, where a concept $A$ is a parent of another concept $B$ if $B \subset A$ and there exists no concept $C$ such that $C\subset A$ and $B \subset C$.
%\end{definition}
%
%As an example, Figure~\ref{fig:conceptDAG} shows a concept-DAG for the clusterings based on `shape'.
%
%\begin{figure}
%	\tiny{\begin{tikzpicture}[%
%		->,
%		>=stealth,
%		node distance=0.3cm,
%		pil/.style={
%			->,
%			thick,
%			shorten =2pt,}
%		]
%		\node (univ) {Universe};
%		\node[below left=of univ] (poly) {Polygons};
%		\node[below left=of poly] (quad) {Qudrilaterals};
%		\node[right=of poly] (nonTri) {Non-triangles};
%		\node[below right=of nonTri] (nonPoly){Round};
%		\node[right=of quad] (tri) {Triangles};
%		\node[below left=of quad] (rect) {Rectangles};
%		\node[right=of rect] (sq) {Squares};
%		\node[right=of sq] (eq) {Equilateral};
%		\node[right=of eq] (scalene) {Scalene};
%		\node[right=of scalene] (circle) {Circles};
%		\node[right=of circle] (ell) {Ellipses};
%		\draw [->] (univ) to (poly);
%		\draw [->] (univ) to (nonTri);
%		\draw [->] (nonTri) to (nonPoly);
%		\draw [->] (nonTri) to (quad);
%		%\draw [->] (univ) to (nonPoly);
%		\draw [->] (poly) to (quad);
%		\draw [->] (poly) to (tri);
%		\draw [->] (nonPoly) to (circle);
%		\draw [->] (nonPoly) to (ell);
%		\draw [->] (quad) to (rect);
%		\draw [->] (quad) to (sq);
%		\draw [->] (tri) to (eq);
%		\draw [->] (tri) to (scalene);
%	\end{tikzpicture}}
%	\caption{\label{fig:conceptDAG}Concept-DAG}
%	
%\end{figure}
%
%\begin{definition}{\bf Hierarchy}
%A {\sc Hierarchy} is a sub-graph of the Concept-DAG (formed by removing concepts) that forms a connected tree and includes the {\tt Universe} concept. Further, every pair of sibling concepts in the hierarchy should have no overlap, and the a complete set of sibling nodes should cover the entire parent concept (with respect to the dataset).
%
%\end{definition}
%
%In the Concept-DAG shown in \ref{fig:conceptDAG}, the concept {\tt Quadrilaterals} has two parents. So we get two possible hierarchies based on which parent of {\tt Quadrilateral} is removed. One of these hierarchies is shown in Figure~\ref{fig:Hier}. Other subgraphs of the concept-DAG are shown in Figures~\ref{fig:notHier1} and \ref{fig:notHier2}. These subgraphs are not hierarchies, even though they form trees. Figure~\ref{fig:notHier2} is not a hierarchy because the concepts of {\tt Polygons} and {\tt Non-Triangles} are not disjoint - A rectangle is a non-triangle that is also a polygon. In Figures~\ref{fig:notHier1}, the concept {\tt Round} does not cover the entire parent concept {\tt Non-triangles} with respect to the dataset and is hence not a hierarchy. The dataset has {\tt Quadrilaterals} in addition to {\tt Round}.
%
%
%\begin{figure*}
%\centering
%\subfigure[][\label{fig:Hier}Hierarchy]{
%        
%	\tiny{\begin{tikzpicture}[%
%		->,
%		>=stealth,
%		node distance=0.3cm,
%		pil/.style={
%			->,
%			thick,
%			shorten =2pt,}
%		]
%		\node (univ) {Universe};
%		\node[below left=of univ] (poly) {Polygons};
%		\node[below left=of poly] (quad) {Qudrilaterals};
%		\node[below right=of univ] (nonPoly){Round};
%		\node[right=of quad] (tri) {Triangles};
%		\node[below left=of quad] (rect) {Rectangles};
%		\node[right=of rect] (sq) {Squares};
%		\node[right=of sq] (eq) {Equilateral};
%		\node[right=of eq] (scalene) {Scalene};
%		\node[right=of tri] (circle) {Circles};
%		\node[right=of circle] (ell) {Ellipses};
%		\draw [->] (univ) to (poly);
%		\draw [->] (univ) to (nonPoly);
%		\draw [->] (poly) to (quad);
%		\draw [->] (poly) to (tri);
%		\draw [->] (nonPoly) to (circle);
%		\draw [->] (nonPoly) to (ell);
%		\draw [->] (quad) to (rect);
%		\draw [->] (quad) to (sq);
%		\draw [->] (tri) to (eq);
%		\draw [->] (tri) to (scalene);
%	\end{tikzpicture}}
%	
%	   }%
%	   \qquad
%	   \subfigure[][\label{fig:notHier1}Not a hierarchy]{
%	\tiny{\begin{tikzpicture}[%
%		->,
%		>=stealth,
%		node distance=0.3cm,
%		pil/.style={
%			->,
%			thick,
%			shorten =2pt,}
%		]
%		\node (univ) {Universe};
%		\node[below left=of univ] (tri) {Triangles};
%		\node[below right=of univ] (nonTri) {Non-triangles};
%		\node[below right=of nonTri] (nonPoly){Round};
%		\node[below left=of tri] (eq) {Equilateral};
%		\node[right=of eq] (scalene) {Scalene};
%		\node[below left=of nonPoly] (circle) {Circles};
%		\node[right=of circle] (ell) {Ellipses};
%		\draw [->] (univ) to (poly);
%		\draw [->] (univ) to (nonTri);
%		\draw [->] (nonTri) to (nonPoly);
%		%\draw [->] (univ) to (nonPoly);
%		\draw [->] (nonPoly) to (circle);
%		\draw [->] (nonPoly) to (ell);
%		\draw [->] (tri) to (eq);
%		\draw [->] (tri) to (scalene);
%	\end{tikzpicture}}
%	}
%		   \qquad
%	   \subfigure[][\label{fig:notHier2}Not a hierarchy]{
%	\tiny{\begin{tikzpicture}[%
%		->,
%		>=stealth,
%		node distance=0.3cm,
%		pil/.style={
%			->,
%			thick,
%			shorten =2pt,}
%		]
%		\node (univ) {Universe};
%		\node[below left=of univ] (poly) {Polygons};
%		\node[below right=of univ] (nonTri) {Non-triangles};
%		\draw [->] (univ) to (poly);
%		\draw [->] (univ) to (nonTri);
%	\end{tikzpicture}}
%	}
%	
%	
%	\caption{\label{fig:hierarchies}Sub-graphs of the Concept-DAG shown in Figure~\ref{fig:conceptDAG} }
%	
%\end{figure*}
%
%\begin{definition}{\bf Frontier}
%A frontier $F$ is a set of concepts $\{C_{1},...,C_{k}\}$ from a hierarchy $\mathcal{T}$ such that
%\begin{enumerate}
%\item $\nexists \ i, j \ \in \ \{1,\cdots , k\} :  C_{i}$ is an ancestor of $C_{j}$ in $\mathcal{T}$
%\end{enumerate}
%\end{definition}
%Intuitively, a frontier is a set of disjoint concepts. Additionally, if a frontier $F$ covers the entire {\tt Universe} of items, we say that $F$ is a \textit{complete frontier}.
%
%\begin{definition}{\bf Complete Frontier}
%A complete frontier $F$ is a set of concepts $\{C_{1},...,C_{k}\}$ that
%\begin{enumerate}
%\item $F$ is a frontier
%\item $\bigcup_{i= 1}^k C_{i} = \text{{\tt Universe}}$
%\end{enumerate}
%\end{definition}
%Thus, a complete frontier represents a valid way of clustering of the set of items. For the hierarchy shown in Figure~\ref{fig:Hier}, \{{\tt Polygons}, {\tt Circles}, {\tt Ellipses}\}, \{{\tt Quadrilaterals}, {\tt Triangles}, {\tt Round}\}, \{{\tt Rectangles}, {\tt Squares}, {\tt Equilateral},{\tt Scalene}, {\tt Circles}, {\tt Ellipses}\} are all complete frontiers and form valid clusterings.
%
%If the workers are not malicious (and do not cluster randomly), it is reasonable to think that they would choose a hierarchy from a fixed (possibly infinite) set of hierarchies. Thereafter, when asked to cluster a set of items, they essentially pick complete frontiers from this hierarchy  and cluster items based on the concepts in the frontier. We additionally assume that workers do not make mistakes, i.e they put the items in the cluster corresponding to the correct concept.
%
%Based on the above discussion, there is thus a one-to-one mapping between concepts in the frontier and clusters provided by the worker. A `concept' can be equivalently represented by the set of items in the dataset that are instances of that concept. We'll refer to concepts as clusters in the ensuing discussion, with the understanding that it is always possible to associate a concept with it.
%
%With an understanding of hierarchies and frontiers, we redefine {\sc Crowd-Clustering} as
%\begin{problem}[Crowd-Clustering Problem]
%Given a task of items, \textsc{Crowd-Clustering Problem} is the task of organizing them into meaningul clusters. These clusters should represent the maximum likelihood frontier in the most likely hierarchy that a worker chooses.
%\end{problem}
%
%At a high-level, our approach to solve the crowd-clustering problem has two stages. In the first stage, we find the most likely hierarchy by asking multiple workers to cluster a small set of items. Once this hierarchy is constructed, we find the most likely frontier on this hierarchy. Thereafter, we ask workers to categorize the remaining items in the dataset into one of the concepts in the frontier. In the next section, we describe the algorithms for finding/constructing the most likely hierarchy using a small set of items. Afterwards, in Section 4, we describe the algorithms for finding the most likely frontier on this hierarchy.

==> references.tex <==
\bibliographystyle{abbrv}
\bibliography{biblio}
